Degeneration of Hodge structures over Picard modular surfaces

We study variations of Hodge structures over a Picard modular surface, and compute the weights and types of their degenerations through the cusps of the Baily-Borel compactification. The main tool is a theorem of Burgos and Wildeshaus.

==> footer.tex <==

\bibliographystyle{alpha}
\selectlanguage{english}  

\bibliography{bibeppe}

\end{document}

